Hindsight Learning for MDPs with Exogenous Inputs

Many resource management problems require sequential decision-making under uncertainty, where the only uncertainty affecting the decision outcomes are exogenous variables outside the control of the decision-maker. We model these problems as Exo-MDPs (Markov Decision Processes with Exogenous Inputs) and design a class of data-efficient algorithms for them termed Hindsight Learning (HL). Our HL algorithms achieve data efficiency by leveraging a key insight: having samples of the exogenous variables, past decisions can be revisited in hindsight to infer counterfactual consequences that can accelerate policy improvements. We compare HL against classic baselines in the multi-secretary and airline revenue management problems. We also scale our algorithms to a business-critical cloud resource management problem -- allocating Virtual Machines (VMs) to physical machines, and simulate their performance with real datasets from a large public cloud provider. We find that HL algorithms outperform domain-specific heuristics, as well as state-of-the-art reinforcement learning methods.

==> parts/relatedwork_longer.tex <==
\section{Related Work}
\label{sec:related_work}

Here we include a brief discussion of salient related work, see \cref{sec:related_work_full} for more details.

\noindent \textbf{Input-Driven MDPs:} Exo-MDPs, the sub-class of MDPs that we consider here, were described in \citet{powell_reinforcement_nodate}.  They characterize sequential decision-making problems as an evolution of \emph{information}, \emph{decision}, \emph{information} sequences.  These models have been considered before with additional assumptions that either the rewards or the transitions factorize so that the exogenous process can be filtered out~\citep{dietterich_discovering_2018,efroni2022sample}. However, they are not suited for Exo-MDPs because filtering out the exogenous process yields demand-agnostic policies, which are highly sub-optimal for resource management problems.

\noindent \textbf{Hindsight Optimization:}
Hindsight optimization has been previously attempted~\cite{chong2000framework,feng2021scalable}, and it is well known that these values are over-optimistic.  \citet{mercier2007performance} show that the regret for hindsight optimization policies can be bound by the hindsight bias, and show for several network scheduling and caching problems that the regret is a constant.  The Progress Hedging (PH) algorithm in \citet{rockafellar1991scenarios} attempts to eliminate this bias by iteratively refining the solution coming from hindsight optimization by adding non-anticipative constraints.  PH has weak guarantees for convergence in non-convex problems (like our settings).  Information relaxation in \citet{brown2021information} extends PH to non-convex and arbitrary reward and action spaces and allows for imperfect penalization of the non-anticipative constraint violations.  These schemes require hand-crafted penalties as well as tractable hindsight planning with those penalized objectives.  From a practical perspective, PH is intractable for the large problem sizes that we consider because of the constraints required.  Another related line of work in \citet{mercier2007performance} similarly foregoes solving for the optimal policy in the empirical MDP with a hindsight learning surrogate, a potentially sub-optimal non-anticipatory policy.  We additionally describe an algorithm to avoid unnecessary computation in large-scale problems by training a policy to imitate it and provide a tighter regret analysis.

\noindent \textbf{RL for OR:} In our work we primarily consider simulations on dynamic Virtual Machine (VM) scheduling.  On the theoretical side, variants of greedy algorithms have been proposed to solve dynamic VM scheduling problems with competitive ratio analysis.  In \citet{stolyar2013infinite} they assume the VM creation requests can be modeled as a Poisson process with lifetimes as an exponential distribution and show that the greedy algorithm achieves the asymptotically optimal policy.  In \citet{li2015dynamic} they develop a hybrid \textsc{FirstFit} algorithm with an improvement on the competitive ratio.  On the more practical side using deep reinforcement learning techniques, in \citet{mao2016resource} they develop a DeepRM system that can pack tasks with multiple resource demands via a policy gradient method.  They also built a job scheduler named DECIMA by modifying actor-critic algorithms with input-driven baselines~\citep{mao2019learning}.  In \citet{zhang2020learning} they solved the heterogeneous scheduling problem with deep $Q$ learning.  Lastly, in \citet{sheng2022learning} they developed SchedRL, a modification of Deep Q Learning with reward shaping to develop a VM scheduling policy.  All of these algorithms modify existing RL algorithms and show empirical gains on variations of the VM scheduling problem.  Our work differs from two perspectives: 1) we consider using hindsight planning explicitly during training time, 2) our algorithms can be applied to any Exo-MDP problems.  We also note that existing deep reinforcement learning has also been applied in other systems applications (without exploiting their Exo-MDP structure) including ride-sharing systems \citep{feng2021scalable}, stochastic queueing networks~\citep{dai2021queueing}, power grid systems~\citep{chen2020powernet}, jitter buffers~\citep{fang2019reinforcement}, and inventory control~\citep{harsha2021math}.

\noindent \textbf{RL for Combinatorial Optimization:} A crucial assumption underpinning our algorithmic framework is the implementation of {hindsight planners} as in \cref{ass:planning_oracle}.  Our framework is well motivated for problems where hindsight planning is efficient, building on the existing optimization literature on solving planning problems~\citep{conforti2014integer,bertsimas1997introduction}.  However, in general these problems as a function of a fixed exogenous input trace can be written as combinatorial optimization problems.  While we consider using hindsight planners for RL problems, a dual lens is using machine learning techniques for combinatorial optimization, as has been explored in recent years \citep{vinyals2015pointer,bello2016neural,chitnis2020learning}.  In particular, in \citet{vinyals2015pointer} they designed a new network architecture and trained using supervised learning for traveling salesman problems.  Similarly in \citet{hu2017solving} they solve variants of online bin packing problems using policy gradient algorithms.  In \citet{tang2020reinforcement} they design novel heuristic branch and bound algorithms using machine learning for integer programming optimization.
